Growing Neoclassical Tearing Modes Seeded via Transient-Induced-Multimode Interactions

Nonlinear extended MHD simulations demonstrating seeding of neoclassical tearing modes (NTMs) via MHD-transient-induced multimode interactions are presented. Simulations of NTMs are enabled by two recent NIMROD code developments: the implementation of heuristic neoclassical stresses and the application of transient magnetic perturbations (MPs) at the boundary. NTMs are driven unstable by the inherently pressure driven kinetic bootstrap current, which arises due to collisional viscosity between passing and trapped electrons. These simulations use heuristic closures that model the neoclassical electron and ion stresses. NTM growth requires a seed island, which is generated by a transiently applied MP in simulations. The capability is demonstrated using kinetic-based reconstructions with flow of a DIII-D ITER Baseline Scenario discharge [R.J. La Haye, et al., Proceedings IAEA FEC 2020]. The applied MP seeds a 2/1 NTM that grows in two phases: a slow growth phase followed by a faster robust growth phase like that observed experimentally. Additionally, an evolving sequence of higher order core modes are excited at first. Power transfer analysis shows that nonlinear interactions between the core modes and the 2/1 helps drive the initial slow growth. Once the induced 2/1 magnetic island reaches a critical width, the NTM transitions to faster robust growth which is well described by the nonlinear modified Rutherford equation. This work highlights the role of nonlinear mode coupling in seeding NTMs.

==> Makefile <==
#
# Version:	$Id: Makefile 1195 2016-11-15 00:46:17Z jking $
#
##########

INPUTFILES = analysis.tex discussion.tex methods.tex preamble.tex appendex.tex intro.tex ntm.bib overview.tex


TITLE	= ntm
MAIN	= ntm
FILES = $(MAIN).tex $(INPUTFILES)

.SUFFIXES: .pdf .tex

SHELL = /bin/bash
ASPELL = `which aspell`

all: $(TITLE).pdf

$(TITLE).pdf:  $(FILES)
	pdflatex $(MAIN)
	pdflatex $(MAIN)
	bibtex $(MAIN)
	pdflatex $(MAIN)
	/bin/cp -f $(TITLE).pdf DraftPDF
	@make findref
	@make findlabel

fast: $(FILES)
	pdflatex $(MAIN)
	/bin/cp -f $(TITLE).pdf DraftPDF

merge: $(FILES)
	@cp $(MAIN).tex temp.tex
	@for file in $(INPUTFILES); do \
	  filebase=`echo $$file | sed "s/.tex//"`; \
	  echo $$file ; \
	  cat temp.tex | sed "s/\\\input{$$filebase}/replaceline/" | awk '$$1=="replaceline" {{system("cat '$$filebase.tex'")} {next}} {print}' > temp2.tex; \
	  mv temp2.tex temp.tex; \
	done
	@cat temp.tex | sed 's|\\bibliography{.*|\\bibliography{merged}|'  > temp2.tex && mv temp2.tex temp.tex
	@cat temp.tex | sed 's|figures\/||' | sed 's|.png||' > DraftTex/$(MAIN)_merged.tex
	@cp $(MAIN).bbl  DraftTex/$(MAIN)_merged.bbl
	@rm -f temp.tex

# Create a bib file with just the cited entries
#exportbib:
#	@bibexport -o DraftTex/merged.bib $(MAIN).aux

spellcheck: jargon.spl
	@echo Spell checking TeX files.
	@if [ -x $(ASPELL) ]; then\
	  for file in $(INPUTFILES); \
	  do  echo ==== $$file;\
	      $(ASPELL) --lang=en --mode=tex --ignore-case --add-extra-dicts ./jargon.spl check $$file;\
	  done; else\
	  echo ASPELL not found.;\
	fi

jargon.spl: jargon.txt
	@echo Updating jargon dictionary.
	aspell --lang=en create master ./jargon.spl < jargon.txt

findref:
	@echo '---------------------------------------------------------'
	@echo Finding undefined references
	@for uref in `grep undefined $(MAIN).log | grep -v There | sed 's/.*\`//g' | sed "s/'.*//g"`; \
	 do  \
		echo "--> $$uref ";\
		grep -n "[rc][ei].*$$uref" *.tex | grep -v '.tex:[0-9]*:%' | grep -v _merged |sed 's/:/ -- Line /' | sed 's/:/:  /';\
		echo ;\
	  done
#	@grep undefined $(MAIN).log | grep -v 'There were'

findlabel:
	@echo '---------------------------------------------------------'
	@echo Finding multiply defined labels:
	@file=$(<) && for mlab in `grep 'multiply defined' $(MAIN).log | grep -v _merged | sed 's/.*\`//g' | sed "s/'.*//g"`; \
	 do  \
		echo "--> $$mlab ";\
		grep -n "label.*$$mlab" *.tex | grep -v _merged;\
		echo ;\
	  done

remake: clean all

clean:
	rm -rf core
	rm -f *~ *.prev *.log *.end *.aux
	rm -f *.bbl *.blg  *.toc *.ps *.pdf
	rm -f $(TITLE).out

realclean: clean
	rm -f *.pdf

.PHONY: full findlabel clean realclean merge exportbib remake findref

